R-GroundBench: A Diagnostic Benchmark for R-Group Groundingin Markush Molecular Editing

Recent advances in AI for scientific discovery enable molecular understandingand design, yet reasoning over incomplete chemical representations remainsunclear.Markush structures, which encode molecular families through variable R-groupplaceholders (\textit{R\textsubscript{1}}, \textit{R\textsubscript{2}}, \textit{X}, etc.), are ubiquitous in pharmaceutical patents and requiregrounding across molecular, textual, and chemical information.However, existing molecule-language benchmarks focus on fully specifiedmolecules, leaving R-group grounding largely unevaluated.We introduce R-GroundBench:, a diagnostic benchmark built from real patent Markushstructures, featuring a Multiple-Choice (VQA) track with controlled difficultyand modality splits, and an open-ended Generation track.Our results reveal a substantial gap between recognition andmolecular grounding.While models achieve over 90\% accuracy on Easy VQA, performance drops to56--66\% on Hard VQA when shortcuts are controlled.Chemical-domain VLMs also remain unreliable, achieving only 25.7--46.2\% on HardVQA despite domain-specific pretraining.Moreover, Generation Exact Match remains below 20\% for most models and below8\% when visual input is required.These findings reveal that current AI systems lack reliable grounding andexecution for Markush editing, highlighting challenges for AI-drivenscientific discovery.

==> latex/tex/dataset.tex <==
% ===========================================================
% 第4章：R-GroundBench 数据集构建
% 结构：
%   4.1 数据来源
%   4.2 Markush 过滤
%   4.3 R-Group 解析与替换
%   4.4 取代基候选池设计
%   4.5 Instruction 生成
%   4.6 分子性质标注
%   4.7 数据集统计
% ===========================================================

\section{\bench{} Construction}
\label{sec:dataset}

% 本章介绍整个 benchmark 的构建流程
% Figure 2 显示完整 pipeline


% ----- 4.1 数据来源 -----
\subsection{Data Source}
\label{sec:dataset:source}

% 数据来自 MolParser-7M 真实专利/文献子集
We source our Markush structures from the \texttt{sft\_real} subset of
MolParser-7M~\cite{molparser}, which contains 91{,}166 molecular image-\esmiles{}
pairs extracted from real patent and literature documents.
This subset provides authentic Markush structures with naturally occurring visual
styles, noise, and annotation diversity---properties absent from purely synthetic
datasets.

% ----- 4.2 Markush 过滤 -----
\subsection{Markush Filtering}
\label{sec:dataset:filter}

% 过滤标准和最终保留数量
We filter samples requiring: at least one standard R-group placeholder
(\texttt{R[1]}--\texttt{R[9]}, \texttt{X}, \texttt{Y}, \texttt{Z}); no
non-standard tokens; at most 10 R-group positions; and RDKit-parseable backbone
SMILES (full criteria in Appendix~\ref{app:filter}).
% 过滤结果
This yields 46{,}727 Markush-containing samples, from which we select
7{,}457 clean samples as the core source. \hl{Applying the instruction
generation pipeline, this expands to
56{,}500 instruction records covering 12{,}962 unique Markush scaffolds.}

% ----- 4.3 R-Group 解析与替换 -----
\subsection{R-Group Parsing and Substitution}
\label{sec:dataset:parse}

% Pipeline 五步走
For each clean Markush sample, we execute a five-step pipeline:
(1)~\textbf{E-SMILES parsing}---extract R-group names and atom indices from the
\texttt{<a>} tokens in the \esmiles{} extension field;
(2)~\textbf{substituent pool selection}---assign a candidate pool to each R-group
position based on the chemical environment of the attachment atom
(Section~\ref{sec:dataset:pool});
(3)~\textbf{substituent sampling}---randomly sample up to 4 distinct combinations
per scaffold;
(4)~\textbf{RDKit substitution and validation}---replace each R-group wildcard with
the sampled substituent SMILES, validate with RDKit, and generate canonical SMILES;
(5)~\textbf{image rendering}---render the edited molecule to a 300$\times$300-pixel
PNG via RDKit's \texttt{Draw.MolToImage}.
% 最终数量
This pipeline produces \hl{55{,}982} unique editing operations across \hl{12{,}962} scaffolds
(mean \hl{4.36} variants per scaffold).

% ----- 4.4 取代基候选池设计 -----
\subsection{Substituent Pool Design}
\label{sec:dataset:pool}
\hl{All substituents are drawn from a curated set of 22 structurally
complex, ring-containing groups (e.g., 4-chlorophenyl, 2-pyridyl,
phenylsulfonyl), organised into seven similarity groups to support
fine-grained discrimination in our VQA difficulty splits.}
\hl{To prevent chemically invalid products, we define three
context-aware sub-pools---a \textbf{halogen-position pool} (7 halogenated
aryl/benzyl groups) for \texttt{X}/\texttt{Y}/\texttt{Z} placeholders,
an \textbf{N-substituent pool} (16 groups) for nitrogen attachment
points, and an \textbf{O-substituent pool} (10 groups) for oxygen
attachment points---each a strict subset of the general pool.}

% ----- 4.5 分子性质标注 -----
\subsection{Property Annotation}
\label{sec:dataset:prop}

% 两类性质来源
\hl{For Advanced tasks, we annotate questions with two categories of properties:}
\paragraph{RDKit-computed physicochemical properties.}
\hl{We compute six molecular descriptors directly from the edited molecule SMILES:} molecular weight (MW), logP
(Wildman-Crippen), topological polar surface area (TPSA), hydrogen bond donors
(HBD), hydrogen bond acceptors (HBA), and rotatable bond count (RotBonds).

\paragraph{Database-derived biological labels.}
We reverse-engineer Markush structures from approved drugs
in ChEMBL~\cite{chembl} (\texttt{max\_phase\,=\,4}), extracting
\hl{two label types:} \textbf{\hl{bioactivity}}
(pIC$\_$50 \hl{values for pairwise potency
comparisons against a shared target) and}
\textbf{\hl{indication/mechanism}}
\hl{(FDA/EMA-approved disease areas and molecular target class).}
The reverse-engineering procedure identifies terminal substituents in approved
drug SMILES, replaces them with wildcard atoms to form Markush scaffolds, and
links to original ChEMBL records (details in Appendix~\ref{app:stats}).

% ----- 4.6 数据集统计 -----
\subsection{Dataset Statistics}
\label{sec:dataset:stats}

%数据集统计
Table~\ref{tab:stats} summarizes the key statistics of \bench{}.
Figure%~\ref{fig:properties} 
reports the physicochemical property 
distributions of edited molecules: molecular weight, heavy atom 
count, LogP, ring count, TPSA, and hydrogen-bond donors all 
follow log-normal profiles consistent with drug-like chemical 
space (mean MW\,=\,428.4\,Da; 70\% of molecules fall in the 
300--700\,Da range).
Figure%~\ref{fig:scaffold} 
shows the Murcko scaffold frequency 
distribution: the high singleton rate and gradually rising 
cumulative coverage curve confirm that no small set of scaffolds 
dominates the dataset, establishing structural diversity across 
the benchmark.
Figure%~\ref{fig:chembl} 
shows the distribution of biological 
targets and pIC$_{50}$ values in the Advanced track: the 308 
SAR clusters span four target classes (Kinase, GPCR, Enzyme, 
Nuclear Receptor) with a near-normal pIC$_{50}$ distribution 
(mean\,=\,6.91, std\,=\,1.19), covering the full pharmacologically 
relevant potency range.

\begin{table}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lp{3.6cm}@{}}
    \toprule
    \textbf{Statistic} & \textbf{Value} \\
    \midrule
    Source subset              & MolParser-7M \texttt{sft\_real} \\
    Raw patent/lit.\ mols      & 91{,}166 \\
    Markush-containing samples & 46{,}727 \\
    Clean samples used         & 7{,}457 \\
    Unique Markush scaffolds   & 12{,}962 \\
    Unique editing operations  & 55{,}982 \\
    Instruction styles         & 2 \\
    Total instruction records  & 56{,}500 \\
    Basic VQA questions        & 940 per split \\
    Advanced VQA questions     & 634 per split \\
    NOTA questions             & about 20$\%$ of Easy/Medium Basic \\
    Generation questions       & 500 easy and 500 hard \\
    Input modalities           & 4 \\
    Mean MW (Da)               & 428.4 \\
    Mean atom count            & 31.4 \\
    ChEMBL SAR clusters        & 308 \\
    Bioactivity data points    & 2{,}390 (mean p\ic{}$_{50}$\,=\,6.91) \\
    Biological labels          & bioactivity, indication, mechanism \\
    \bottomrule
  \end{tabular}
  \caption{\bench{} dataset statistics after filtering and validation.}
  \label{tab:stats}
\end{table}




==> latex/tex/task.tex <==
% ===========================================================
% §3 Task and Benchmark Design
% 合并原 §3 Task Definition + §5 Diagnostic Benchmark Design
% 结构：
%   3.1 形式化定义
%   3.2 Basic and Advanced Tasks
%   3.3 输入-输出模态
%   3.4 Easy vs. Hard Splits
%   3.5 None-of-the-Above (NOTA)
%   3.6 Evaluation Metrics
% ===========================================================
 
\section{Task and Benchmark Design}
\label{sec:task}
\begin{figure*}[thb]
  \centering
  \includegraphics[width=0.85\linewidth]{latex//fig/framework.png}
  \caption{%
    Joint overview of task formalization (\S\ref{sec:task}) and dataset
    construction (\S\ref{sec:dataset}).
    \textbf{Panel A}: the construction pipeline---MolParser-7M scaffolds are
    filtered for validity, paired with context-aware substituent pools (15 common
    groups for Easy/Medium; 27 complex ring-containing groups for Hard), and
    processed through reverse engineering of ChEMBL approved drugs for Advanced
    tasks; five instruction templates yield diverse task instances.
    \textbf{Panel B}: the benchmark design---formal task definition
    ($X=(x_s, x_i)\to Y$), two core task types (Basic targeted substitution and
    Advanced property-guided generation), three diagnostic difficulty splits
    (Easy/Medium/Hard) with progressively constrained distractors, four
    cross-modal input-output settings, and NOTA robustness testing (20\% of VQA
    questions).
  }
  \label{fig:framework}
\end{figure*}
% ----- 3.1 形式化任务定义 -----
\subsection{Formal Definition}
\label{sec:task:formal}

Let $M$ denote a Markush representation, which may be either a molecular image
$M_\text{img}$ or an \esmiles{} string $M_\text{smi}$.
An \esmiles{} string extends standard RDKit SMILES with a \texttt{<sep>} delimiter
and an extension field that encodes R-group positions via XML-like tokens:
\begin{center}
  \footnotesize
  \texttt{N1=CC(*)=C(*)N=C1*<sep>}\\
  \texttt{<a>3:R[1]</a><a>5:R[2]</a><a>8:X</a>}
\end{center}
Given $M$, a natural-language instruction $I$, and a candidate set
$\mathcal{C} = \{C_1, C_2, C_3, C_4\}$ where each $C_k$ is a molecule image
or SMILES string, the model must select the candidate $C^*$ corresponding to
the molecule obtained by grounding the specified R-group placeholder and
substituting it with the correct substituent:
\begin{equation}
  C^* = \arg\max_{C_k \in \mathcal{C}}\; P(C_k \mid M, I).
  \label{eq:task}
\end{equation}
When none of the candidates is correct (\emph{none-of-the-above} cases), the
model should output the special answer ``None of the above.''

% ----- 3.2 Basic and Advanced Tasks -----
\subsection{Basic and Advanced Tasks}
\label{sec:task:types}

\paragraph{Basic R-Group Editing.}
In the \textbf{Basic} task, the instruction $I$ directly names the substituent:
\begin{quote}
  \small\itshape
  ``Replace R\textsubscript{1} with 4-chlorophenyl.''
\end{quote}
\hl{The model must localize the specified placeholder in $M$, identify the
named substituent, and select the candidate $C^*$ that reflects the correct
structural edit.}
Basic tasks probe R-group localization and substituent recognition in the
absence of property reasoning.

\paragraph{Advanced Property-Guided Editing.}
In the \textbf{Advanced} task, $I$ poses a property-based question rather than
naming a specific substituent:
\begin{quote}
  \small\itshape
  ``Which R-group substitution gives the highest molecular weight?''\\
  ``Which molecule has been approved for the treatment of rheumatoid arthritis?''
\end{quote}
Property questions span three categories:
\textbf{Physicochemical} (25\%: MW, logP, TPSA, HBD, HBA, rotatable bonds,
computed by RDKit),
\textbf{Biological activity} (45\%: potency comparisons based on
IC\textsubscript{50} values from ChEMBL), and
\textbf{Indication/Mechanism} (30\%: approved drug indications and mechanisms
of action from ChEMBL).
\hl{Advanced tasks require structure-to-property reasoning on top of
structural recognition; their difficulty stems from property knowledge
rather than distractor design, as confirmed by the near-zero
$\Delta_{\text{EH}}$ observed across Advanced splits in our experiments.}

% ----- 3.3 输入-输出模态 -----
\subsection{Input-Output Modalities}
\label{sec:task:modality}

To disentangle visual perception, symbolic manipulation, and cross-modal
alignment, \bench{} covers four input-output modality combinations
(Table~\ref{tab:modalities}).
Text-only LLMs are evaluated solely under the \textbf{smi-smi} setting;
VLMs are evaluated across all four settings, enabling us to attribute performance
differences to visual perception failures, symbolic reasoning failures, or
cross-modal alignment failures.

\begin{table}[htb]
  \centering
  \scriptsize
  \begin{tabular}{llll}
    \toprule
    \textbf{Mode} & \textbf{Input} & \textbf{Candidates} & \textbf{Tests} \\
    \midrule
    img-img & Markush image & mol.\ images   & Visual grounding \\
    img-smi & Markush image & SMILES options & Image$\to$symbol \\
    smi-img & \esmiles{}    & mol.\ images   & Symbol$\to$visual \\
    smi-smi & \esmiles{}    & SMILES options & Symbolic editing \\
    \bottomrule
  \end{tabular}
  \caption{The four input-output modality settings in \bench{},
           each isolating a distinct aspect of multimodal R-group grounding.}
  \label{tab:modalities}
\end{table}

% ----- 3.4 Easy vs. Hard Splits -----
\subsection{Easy vs.\ Medium vs.\ Hard Splits}
\label{sec:task:splits}

A na\"{i}ve multiple-choice setup can yield artificially inflated accuracy:
cross-scaffold candidates betray the answer without R-group parsing, substituent
name tokens correlate with candidate labels, and visual size differences provide
shortcuts.
To control for these confounds, we design \hl{three} 
complementary difficulty levels \hl{that isolate the effect of 
distractor composition and instruction style as independent 
variables}
(Table~\ref{tab:splits}).

\begin{table}[t]
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lp{3.0cm}p{1.8cm}}
    \toprule
    \textbf{Split} & \textbf{Distractor design} & \textbf{Instruction style} \\
    \midrule
    Easy   & Cross-scaffold: different backbones
           & Direct name \\[4pt]
    Medium & Same-scaffold: identical backbone
           & Direct name \\[4pt]
    Hard   & Same-scaffold: highest Tanimoto similarity
           & Descriptive \\
    \bottomrule
  \end{tabular}
  \caption{%
    \hl{Three-level diagnostic split design. Each level independently
    controls distractor composition and instruction style.}
  }
  \label{tab:splits}
\end{table}

\paragraph{Easy split.}
Candidates are drawn from \emph{different} Markush scaffolds.
Instructions use direct substituent names (e.g., ``Replace R\textsubscript{1}
with 4-chlorophenyl'').
\hl{The cross-scaffold shortcut allows a model to identify the correct answer
by backbone similarity alone, without genuinely grounding the R-group edit.}

\paragraph{Medium split.}
\hl{All four candidates share the \emph{same} Markush scaffold and
differ only in the substituent occupying each R-group position,
removing the cross-scaffold shortcut present in Easy splits.
Instructions retain direct substituent names, isolating the
effect of distractor composition from instruction style.}

\paragraph{Hard split.}
All four candidates share the \emph{same} Markush scaffold;
distractors are the three same-scaffold variants most similar to
the correct answer by ECFP4 Tanimoto similarity, maximally reducing
visual discriminability.
Instructions use \emph{only} descriptive paraphrases
(e.g., ``a six-membered nitrogen-containing aromatic ring'' for pyridyl),
requiring structural interpretation rather than name matching.
\hl{Hard splits contain no NOTA questions.}




% ----- 3.5 None-of-the-Above (NOTA) -----
\subsection{None-of-the-Above (NOTA) Questions}
\label{sec:task:nota}

Real-world Markush editing can fail---the specified R-group may not exist in the
scaffold, or none of the candidates may match the instruction.
To test whether models can \emph{reject} invalid options, 20\% of Basic questions
include a NOTA choice: 5\% where the correct answer is among A/B/C (testing
robustness to NOTA as a distractor); 10\% where all of A/B/C contain subtle
structural errors, making NOTA correct; and 5\% where the instruction references
a non-existent R-group.
We report NOTA accuracy separately to assess calibration.

% ----- 3.6 Evaluation Metrics -----
\subsection{Evaluation Metrics}
\label{sec:task:metrics}

\paragraph{VQA.}
We report \textbf{split-wise accuracy} for each of the six splits and
\textbf{property-type accuracy} for Advanced tasks, disaggregated into
physicochemical, bioactivity, and indication/mechanism categories.
The Easy$\to$Hard gap ($\Delta_\text{EH}$ = Easy $-$ Hard) and NOTA
accuracy are reported as defined in \S\ref{sec:task:splits}
and~\S\ref{sec:task:nota}, respectively.
To mitigate answer-position bias, correct answers are uniformly distributed
across A/B/C/D and candidate order is randomized per instance.

\paragraph{Generation.}
\hl{We evaluate open-ended SMILES output with three complementary metrics:
\textbf{Exact Match (EM)}, the strictest measure, requires the predicted
SMILES (after RDKit canonicalization) to be identical to the ground truth;
\textbf{Scaffold Match} checks whether the predicted molecule retains the
core Markush backbone via MCS coverage; and
\textbf{Tanimoto Similarity} (ECFP4, range 0--1) captures partial structural
overlap when EM fails.
Together they distinguish complete correctness, backbone retention, and
approximate similarity---three qualitatively different failure modes.}
